Future-Dependent Value-Based Off-Policy Evaluation in POMDPs

We study off-policy evaluation (OPE) for partially observable MDPs (POMDPs) with general function approximation. Existing methods such as sequential importance sampling estimators and fitted-Q evaluation suffer from the curse of horizon in POMDPs. To circumvent this problem, we develop a novel model-free OPE method by introducing future-dependent value functions that take future proxies as inputs. Future-dependent value functions play similar roles as classical value functions in fully-observable MDPs. We derive a new Bellman equation for future-dependent value functions as conditional moment equations that use history proxies as instrumental variables. We further propose a minimax learning method to learn future-dependent value functions using the new Bellman equation. We obtain the PAC result, which implies our OPE estimator is consistent as long as futures and histories contain sufficient information about latent states, and the Bellman completeness. Finally, we extend our methods to learning of dynamics and establish the connection between our approach and the well-known spectral learning methods in POMDPs.

==> finite_horizon.tex <==
\section{Finite Horizon}
\masa{not yet}
\subsection{Problem Setting}

The data is generated by executing a set of policies $\pi= \{\pi_t\}$ where $\pi_t:\Ucal_t \times \Ocal \to \Delta(\Acal)$ where $\Ucal_t = \otimes_{k=0}^{t-1} \{\Ocal \times \Acal \times [0,1] \}$. Here, $\Ucal_t$ denotes the all history before observing an observation at time step $t$.
Given an initial distribution $\nu_S \in \Delta(\Acal)$ and a policy $\pi$, the data generating process is summarized as $S_0 \sim \nu_S, O_0 \sim Z_0(\cdot \mid S_0), A_0\sim \pi_0(\cdot \mid O_0),R_0 = r_0(S_0,A_0),\cdots,A_t \sim \pi_t(\cdot \mid U_t,O_t),\cdots$. Comparing to standard MDPs, we cannot directly observe the latent state $S_t$. Instead, we have access to an observation $O_t$. We denote its distribution by $P_{\pi}$. The policy value is defined as the expected cumulative reward $\EE_{\pi}[\sum_{t=0}^{T-1}\gamma^tR_t]$ for some $0<H\leq +\infty$ where the expectation is taken with respect to the distribution of trajectories induced by policy $\pi$. 




The goal of OPE is to estimate $J(\pi^e)$ from an offline dataset $\Dcal$ that consists of $N$ data trajectories, generated by a behavior policy $\pi^b = \{\pi^b_t\}_t$. By using sequential importance sampling,  we can easily identify this value from the offline data: 
\begin{align*}
    \EE\left[ \sum_{t=0}^{T-1}  \gamma^t \nu_t R_t  \right],\nu_t = \prod_{k=0}^t \mu_t, \mu_t= \frac{\pi^e_t(A_t \mid U_t, O_t)}{\pi^b_t(A_t \mid U_t, O_t)}, 
\end{align*}
where the expectation without subscript is taken with respect to the distribution of trajectories induced by policy $\pi^b$.  The estimator is then constructed by $\hat J_{\SIS}=\EE_{\Dcal}\left[ \sum_{t=0}^{\infty}  \gamma^t \nu_t R_t  \right].$
where $\EE_{\Dcal}$ denotes the sample average over offline data. While this estimator is unbiased,  the variance of estimators grows exponentially with respect to the horizon. Our goal is to propose estimators which overcome these this challenge.  

Before proceeding our proposal, we stream the notation as follows. We define two random variables: $U_t=(O_0,A_0,R_0\cdots, A_{t-1},R_{t-1}),U'_t =(O_t,A_t,R_t,\cdots,O_{T-1}) $. Here, $U_t$ is a set of all history variables and $U'_t$ is a set of all future random variables. Let $F_t,\bar H_t$ be some subsets of $U_t,U'_t$, respectively. We denote their domains by $\Fcal_t,\bar \Hcal_t$, respectively. We suppose $\pi^e_t,\pi^b_t$ only depend on $\bar H_t$. For the ease of exposition, we suppose $\bar H_t=U_{t}$ for $0\leq t\leq M$ and $\bar H_t =(A_{t-M},O_{t-M},R_{t-M},\cdots,A_{t-1},O_{t-1},R_{t-1})$. 
In other words, $\pi^e,\pi^b$ are $m$-memory policies. We also define another subset $\bar H_t$ such that $\bar H_t \subsetneq H_t \subset U_t$ which include $\bar H_t$ for $t\leq M$. We further denote $\bar F_t = (\bar H_t,F_t), \bar S_t=(\bar H_t,S_t)$ and denote their domains by $\bar \Fcal_t,\bar \Scal_t$. We denote $\Dcal = \{U^{[i]}_T\}_{i=1}^n$. Given a policy $\pi$, we define the state value function at time step $t$, $V^{\pi}_t(\bar s)=\EE_{\pi}[\sum _{k=t}^{T-1} \gamma^t R_t \mid \bar S_t=\bar s]$ for $\bar s\in \bar \Scal_t$. 



==> main_alternative.tex <==
\section{Alternative Sufficient Conditions }\label{sec:alternative}






In this section, we present sufficient conditions to estimate policy values, which are different from those in \pref{sec:relaxed}. 

\subsection{With the Existence of Future-dependent weight Functions in place of Invertibiilty Conditions}

We have so far assumed the invertibility condition in \pref{thm:identify2}. We can replace it with another condition. To do that, we introduce future-dependent weight functions. 

\begin{definition}[Future-dependent weight functions]
Future-dependent weight functions $g_W(\cdot):\Hcal \to \RR$ are defined as solutions to the solution to the following integral equation: 
\begin{align*}
    \EE[g_W(H) \mid Z,S]=w_{\pi^e}(Z,S). 
\end{align*}
We denote the set of solutions by $\Gcal_W$. 
\end{definition}
This is an embedding of marginal ratios onto the observation space. By using $g_W(\cdot)$ implicitly, we can identify the policy value.  

\begin{theorem}[Identification with future-dependent weight functions]\label{thm:weight}
Suppose (\ref{thm:weight}a) learnable future-dependent value functions exist, (\ref{thm:weight}b) weight future-dependent value functions exist,  (\ref{thm:weight}c) the overlap $w_{\pi^e}(Z,S)<\infty,\mu(Z,O,A)<\infty$. Then, for any $b_V \in \Bcal_V$, we have 
\begin{align*}
    J(\pi^e) = \EE_{\bar f\sim \nu_{\bar F}}[b_V(\bar f)]. 
\end{align*}
\end{theorem}

Compared to \pref{thm:identify2}, we suppose the existence of future-dependent weight functions in place of the invertibility. The existence of future-dependent weight functions requires that the history except for the $M$-memory, i.e., $H \setminus (Z)$ retains sufficient information about $S$. Thus, it shares the same spirit of the invertibility condition. The shortcoming of this strategy is we always need the overlap in terms of density ratio and we cannot refine the coverage concept as in (\ref{thm:identify2}c). In the tabular case, exactly same assumptions ensure (a) and (b) in \pref{thm:weight}. 

\begin{myexp}[continues=exa:tabular] 
Consider tabular models. The existence of future-dependent weight functions is satisfied when $\Prr_{\pi^b}(\Hb \mid \bar \Sbb_b ) = |\bar \Scal_b|$. Note this is equivalent to   $\Prr_{\pi^b}(\bar \Sbb_b, \Hb ) = |\bar \Scal_b|$ in \pref{lem:equivalent}. 
\end{myexp}


\subsubsection{Finite Sample Result}

Elaborating on \pref{thm:weight}, we have the following finite-sample result. 

\begin{theorem}[Finite sample version of \pref{thm:weight}] \label{thm:finite_weight}

Set $\lambda =0$. Suppose (\ref{thm:weight}a), (\ref{thm:weight}b), (\ref{thm:weight}c) in \pref{thm:weight}. Assume we have realizability $\Gcal \cap \Bcal_V \neq 0$ and $\Xi \cap \Gcal_W \neq 0$. Then, 
\begin{align*}
    |J(\pi^e) - \hat J_{\mathrm{VM}}|\leq c(1-\gamma)^{-2}\max(1,C_{\Qcal},C_{\Xi})^2\sqrt{\ln(|\Qcal| |\Xi| /\delta)/n }. 
\end{align*}
\end{theorem}


\subsection{Without Bellman Completeness Assumptions} \label{subsec:without_bellman}

We have assumed the Bellman completeness  $\Tcal \Qcal \subset \Xi$ in \pref{sec:relaxed}. We can replace this condition with another condition. 


Firstly, we introduce $\Xi$-learnable future-dependent value functions instead of learnable future-dependent value functions.  



\begin{definition}[$\Xi$-learnable future-dependent value functions]
$\Xi$-learnable future-dependent value functions are defined as solutions to 
\begin{align*}
   \sup_{\xi \in \Xi }|\EE[(\mu(Z,O,A)\{R + \gamma b_V(\bar F')\} - b_V(\bar F)) \xi(H) ]|=0. 
\end{align*}
We denote the set of solutions by $\Bcal^{\Xi}_V$. 
\end{definition}

Note we have $\Bcal^{\Xi}_V \subset \Bcal_V$. Thus, the existence of $\Xi$-learnable future-dependent value functions is weaker than the one of learnable future-dependent value functions. %

With the above preparation in our mind, we present a refined identification formula.  




\begin{theorem}[Refined identification theorem ver 2] \label{thm:identify3}
Suppose (\ref{thm:identify3}a) $\Bcal^{\Xi}_V \cap \Qcal \neq \emptyset$, (\ref{thm:identify3}b) any element in $q \in \Qcal $ that satisfies $\sup_{\xi \in \Xi}|\EE[\Tcal^{S}(q)(\bar S)\xi(H)]|=0 $ satisfy $\Tcal^{S}(q)(\bar S) =0$,  
(\ref{thm:identify3}c) overlap, the same as (\ref{thm:identify2}c). For any $b_V \in\Bcal^{\Xi}_V\cap\Qcal $, we have 
     \begin{align}
         J(\pi^e) = \EE_{\bar f \sim \nu_{\bar \Fcal}}[b_V (\bar f) ]. 
    \end{align}
\end{theorem}

The condition (\ref{thm:identify3}a) is a realizability assumption weaker than (\ref{thm:identify2}a) while the condition (\ref{thm:identify3}b) is stronger than (\ref{thm:identify2}b). 
The advantage of this approach compared to \pref{thm:identify2} is that we do not directly need the Bellman completeness since we can identify some element in $\Bcal^{\Xi}_V \cap \Qcal$ from the loss function \pref{eq:full}. This type of condition without Bellman completeness is known in OPE with linear models as well \citep{uehara2020minimax,perdomo2022sharp}. In fact, this advantage is clearly seen when we instantiate the theorem on LQG. 

\begin{myexp}[continues=exa:hse_pomdps]
Consider HSE-POMDPs with linear models. Using \pref{thm:identify3}, we get the following lemma. 

\begin{lemma}[Formula for HSE-POMDPs]\label{lem:refined_hse}
Suppose (LM1)-(LM4),(LM7), and (LMW5): 
\begin{align*}
    \sup_{x \in \RR^d, x^{\top}\EE[\phi_{\bar \Scal}(\bar S)\phi^{\top}_{\Hcal}(H) ]\EE[\phi_{\Hcal}(H)\phi^{\top}_{\bar \Scal}(\bar S) ]x \neq 0} \frac{x^{\top}\EE[\phi_{\bar \Scal}(\bar S)\phi_{\bar \Scal}(\bar S)^{\top}] x }{x^{\top}\EE[\phi_{\bar \Scal}(\bar S)\phi^{\top}_{\Hcal}(H) ]\EE[\phi_{\Hcal}(H)\phi^{\top}_{\bar \Scal}(\bar S) ] x } < \infty. 
\end{align*}
Then, we have 
\begin{align*}
  J(\pi^e) = \EE_{\bar f \sim \nu_{\bar \Fcal}}[\phi_{\bar \Fcal}(\bar f)]^{\top}\EE[\phi_{\Hcal}(H)\{\phi_{\bar \Fcal}(\bar F)-\gamma \mu(Z,O,A)\phi_{\bar \Fcal}(\bar F')\}^{\top} ]^{+}\EE[\mu(Z,O,A)R \phi_{\Hcal}(H)]. 
\end{align*}
\end{lemma}

Compared to \pref{lem:lqg}, we do not require (LM6), which is the existence of conditional mean embedding operator between $\bar S$ and $H$ while we instead require (LMW5), which is stronger than (LM5). 



\end{myexp}


\subsubsection{Finite Sample Result}

Elaborating on \pref{thm:identify3}, we have the following finite-sample result. 

\begin{theorem}[Finite sample version of \pref{thm:identify3}] \label{thm:finite_identify3}
Set $\lambda>0$. Suppose (\ref{thm:identify3}a), (\ref{thm:identify3}b), (\ref{thm:identify3}c).  With probability $1-\delta$,  we have 
\begin{align}\label{eq:first}
    |J(\pi^e) - \hat J_{\VM}| &\leq  c(1-\gamma)^{-2}(1/\lambda + \lambda)\max(1,C_{\Qcal}, C_{\Xi})\kappa_2(\Qcal)  \sqrt{\frac{\ln (  |\Qcal| |\Xi|c /\delta)}{n} }, \\
    \kappa^2_2(\Qcal) &:= \sup_{q \in \Qcal,  \sup_{\xi \in \Xi }\EE[ \Tcal^{\Scal}(q)(\bar S) \xi(H) ]^2\neq 0 } \frac{ \EE_{\bar s \sim d_{\pi^e}}[(\Tcal^{S}q)^2(\bar s) ]}{  \{\sup_{\xi \in \Xi }\EE[ \Tcal^{\Scal}(q)(\bar S) \xi(H) ]^2\}}. \nonumber 
\end{align}
Here,  note $ \kappa_2(\Qcal) \leq  \mathrm{Dr}_{\Qcal}(d_{\pi^e},P_{\pi^b}) \mathrm{IV}_2(\Qcal,\Xi)$ where 
\begin{align*}
    \mathrm{IV}_2(\Qcal,\Xi) <\infty\,\,\textrm{where}\,\, \mathrm{IV}_2(\Qcal,\Xi):= \sup_{q\in \Qcal, \sup_{\xi \in \Xi }\EE[ \Tcal^{\Scal}(q)(\bar S) \xi(H) ]^2 \neq 0 }\frac{\EE[\{\Tcal^{\Scal}(q)\}^2(\bar S)]  }{ \{\sup_{\xi \in \Xi }\EE[ \Tcal^{\Scal}(q)(\bar S) \xi(H) ]^2\}  }. 
\end{align*}
\end{theorem}

Here, the non-vacuous PAC guarantee is ensured when $\mathrm{Dr}_{\Qcal}(d_{\pi^e},P_{\pi^b})<\infty$, which corresponds to the overlap in (\ref{thm:identify3}c), and $\mathrm{IV}_2(\Qcal,\Xi)<\infty$, which corresponds to  (\ref{thm:identify3}b). Thus, we do not require the Bellman completeness anymore. 

==> proof.tex <==


\section{Proof of \pref{sec:identification}}

\subsection{Proof of \pref{lem:helpful}}

From the Bellman equation, we have 
\begin{align*}
    0 &=  \EE_{\pi^e}[\{R_t + \gamma V^{\pi^e}_{t+1}(\bar H_{t+1},S_{t+1}) \} - V^{\pi^e}_{t}(\bar H_{t},S_{t})  \mid \bar H_t,S_t ]\\
     &= \EE[\mu_t(\bar H_t,A_t,O_t)\{R_t + \gamma V^{\pi^e}_{t+1}(\bar H_{t+1},S_{t+1}) \} - V^{\pi^e}_{t}(\bar H_{t},S_{t})  \mid \bar H_t,S_t ].  
\end{align*}
Then, following the definition of value bridge functions, we immediately have   
\begin{align*}
 & \EE[\mu_t(\bar H_t,A_t,O_t)\{R_t + \gamma g^{[t+1]}_V(H_{t+1},F_{t+1}) \} \mid \bar H_t,S_t ] \\ 
   &= \EE[\mu_t(\bar H_t,A_t,O_t)\{R_t + \gamma \EE[g^{[t+1]}_V(H_{t+1},F_{t+1})\mid  \bar H_{t+1},S_{t+1}] \} \mid \bar H_t,S_t ] \tag{$F_{t+1} \perp (A_t,O_t,R_t,\bar H_t)\setminus \bar H_{t+1}  \mid \bar H_{t+1},S_{t+1}$}\\ 
   &=\EE[\mu_t(\bar H_t,A_t,O_t)\{R_t + \gamma V^{\pi^e}_{t+1}(\bar H_{t+1},S_{t+1}) \} \mid \bar H_t, S_t] \\
   &=V^{\pi^e}_{t}(\bar H_{t},S_{t}) \tag{Bellman equations}\\ 
   &= \EE[g^{[t]}_V(\bar H_t,F_{t}) \mid \bar H_t,S_t ].   \tag{Definition}
\end{align*}
Finally, since $F_t \perp (H_t\setminus \bar H_t ) \mid \bar H_t,S_t$, 
we have 
\begin{align*}
    &\EE[\mu_t(\bar H_t,A_t,O_t)\{R_t + \gamma g^{[t+1]}_V(H_{t+1},F_{t+1}) \} -g^{[t]}_V(H_t,F_{t}) \mid H_t ]\\
    &=\EE[\EE[\mu_t(\bar H_t,A_t,O_t)\{R_t + \gamma g^{[t+1]}_V(H_{t+1},F_{t+1}) \} -g^{[t]}_V(H_t,F_{t})\mid \bar H_t,S_t ]\mid H_t ]\\
    &=0. 
\end{align*}

\subsection{Proof of  \pref{thm:identify} }

We prove two proofs. In the first proof, we directly concludes the final statement. In the second proof, as an intermidiate step, we show learnable value bridge functions are bridge functions. 

\paragraph{Direct Proof of Identification }
We have 
\begin{align*}
   &J(\pi_e) =   \EE[\sum_{t=0}^{H-1}  \gamma^t\nu_t R_t]  =   \EE[\sum_{t=0}^{H-1}\EE[ \nu_{t-1} \mid  \bar H_t,S_t]  \mu_t(\bar H_t,O_t,A_t) \gamma^t R_t] \tag{$(U_{t} \setminus \bar H_t )  \perp A_t,R_t,O_t \mid S_t,\bar H_t$} \\ 
         &=   \EE[\sum_{t=0}^{H-1} \gamma^t \EE[ \nu_{t-1} \mid  \bar H_t,S_t]\EE[  \mu_t(\bar H_t,O_t,A_t) R_t \mid \bar H_t, S_t]]. 
 \end{align*}  
Here, we have
 \begin{align}\label{eq:direct_result}
  \EE[ \mu_t\{\gamma b^{[t+1]}_V(\bar H_{t+1},F_{t+1})+  R_t\}-b^{[t]}_V(\bar H_t,F_t) \mid \bar H_t, S_t]=0. 
 \end{align}
 since 
 \begin{align*}
      &\EE[ \mu_t\{\gamma b^{[t+1]}_V(\bar H_{t+1},F_{t+1})+  R_t\}-b^{[t]}_V(\bar H_t,F_t) \mid H_t]\\
      &=  \EE[ \EE[ \mu_t\{\gamma b^{[t+1]}_V(\bar H_{t+1},F_{t+1})+  R_t\}-b^{[t]}_V(\bar H_t,F_t)\mid \bar H_t,S_t] \mid H_t]
 \end{align*}
 and the completeness assumption. Thus, 
{\small 
 \begin{align*}
     &J(\pi_e)  =  \sum_{t=0}^{H-1} \gamma^t \EE[\EE[ \nu_{t-1}\mid  \bar H_t,S_t]\{- \EE[\mu_t(\bar H_t,O_t,A_t)\gamma b^{[t+1]}_V(\bar H_{t+1},F_{t+1})+ b^{[t]}_V(\bar H_t,F_t)  \mid \bar H_t, S_t] \} ]  \\ 
     &= \EE[b^{[0]}_V(F_0)  ] +\\
         & \sum_{t=0}^{H-1} \EE \bracks{ -\EE[ \nu_{t-1} \mid  \bar H_t,S_t] \EE[\mu_t(\bar H_t,O_t,A_t)\gamma b^{[t+1]}_V(\bar H_{t+1},F_{t+1}) \mid \bar H_t, S_t] + \gamma\EE[ \nu_{t+1} \mid  \bar H_{t+1}, S_{t+1}] \EE[b^{[t+1]}_V(\bar H_{t+1},F_{t+1})  \mid \bar H_{t+1}, S_{t+1}]  } \tag{Telescoping sum} \\ 
    &= \EE[b^{[0]}_V(F_0)  ] \\
         & +\sum_{t=0}^{H-1} \EE\bracks{-\EE[ \nu_{t-1} \mid  \bar H_t,S_t] \mu_{t}(\bar H_t,A_t,O_t)\gamma b^{[t+1]}_V(\bar H_{t+1},F_{t+1})  +  \gamma\EE[ \nu_{t} \mid  \bar H_{t+1}, S_{t+1}] b^{[t+1]}_V(\bar H_{t+1},F_{t+1})   } . 
\end{align*}
}
Here,
\begin{align*}
    & \EE[\EE[ \nu_{t-1} \mid  \bar H_t,S_t] \mu_{t}(\bar H_t,A_t,O_t) b^{[t+1]}_V(\bar H_{t+1},F_{t+1})] \\
    &= \EE[ \nu_{t-1}(U_{t-1})  \mu_{t}(\bar H_t,A_t,O_t) b^{[t+1]}_V(\bar H_{t+1},F_{t+1})] \tag{ 
    $(U_{t} \setminus \bar H_t) \perp A_t,O_t,F_{t+1} \mid S_t,\bar H_t $ } \\
      &= \EE[ \nu_{t}(U_{t})  b^{[t+1]}_V(\bar H_{t+1},F_{t+1})]\\
      &=\EE[\EE[ \nu_{t} \mid  \bar H_{t+1}, S_{t+1}] b^{[t+1]}_V(\bar H_{t+1},F_{t+1})   ].  \tag{ $ (U_{t} \setminus \bar H_{t+1}) \perp  F_{t+1} \mid  \bar H_{t+1}, S_{t+1} $}  
\end{align*}
Thus, $J(\pi_e) = \EE[b^{[0]}_V(F_0)  ] $. 

\paragraph{Indirect Proof of Identification }

We prove learnable value bridge functions are value bridge functions. We use induction. Consider $b^{[H-1]}_V$. Then, from the completeness, this is a value bride function. Next, consider some time step $t$ for $0<t<H-1$ assuming learnable value bridge functions are value bridge functions from time steps $t+1$ to $H$.  

First, from the completeness, following \pref{eq:direct_result}, we have
\begin{align*}
    \EE[b^{[t]}_V(\bar H_{t},F_{t})\mid  \bar H_t,S_t ]=\EE[\mu_t(\bar H_t,O_t,A_t)\{R_t+ \gamma b^{[t+1]}_V(\bar H_{t+1},F_{t+1})\} \mid \bar H_t, S_t  ]. 
\end{align*}
Then, 
\begin{align*}
     & \EE[b^{[t]}_V(\bar H_{t},F_{t})\mid  \bar H_t,S_t ]\\
     &= \EE[\mu_t(\bar H_t,O_t,A_t)\{R_t+ \gamma b^{[t+1]}_V(\bar H_{t+1},F_{t+1})\} \mid \bar H_t, S_t  ] \\
    &= \EE[\mu_t(\bar H_t,O_t,A_t)\{R_t+ \gamma \EE[ b^{[t+1]}_V(\bar H_{t+1},F_{t+1}) \mid \bar H_{t+1},S_{t+1}]\} \mid \bar H_t, S_t  ] \tag{$F_{t+1} \perp  (\bar H_t,O_t,A_t) \setminus \bar H_{t+1}  \mid S_{t+1},\bar H_{t+1}$ }  \\ 
       &= \EE[\mu_t(\bar H_t,O_t,A_t)\{R_t+ \gamma V^{\pi^e}_{t+1}(\bar H_{t+1},S_{t+1})\} \mid \bar H_t, S_t  ] \tag{Definition}  \\ 
            &=V^{\pi^e}_{t}(\bar H_{t},S_{t}). 
\end{align*}
This implies $b^{[t]}_V$ is a value bridge function. Thus, $b^{[j]}_V$ is a value bridge function for any $0\leq j\leq T-1$. 

Finally, 
\begin{align*}
    J(\pi_e) = \EE[b^{[0]}_V(F_0)  ] 
\end{align*}
is immediately concluded by $    J(\pi_e) = \EE[g^{[0]}_V(F_0)  ] $. 

\subsection{Proof of \pref{lem:tabular}}

The existence of bridge functions is ensured by 
\begin{align}\label{eq:rank1}
    \rank( \Prr(\bar \Fb_t \mid \bar \Sbb_t ) )=|\bar \Scal_t|. 
\end{align}
From \pref{lem:helpful}, this ensures the existence of value bridge functions. 
The completeness is ensured by 
\begin{align}\label{eq:rank2}
    \rank( \Prr(\bar \Sbb_t \mid \Hb_t ) )=|\bar \Scal_t| .
\end{align}
Thus, these two conditions are sufficient conditions. 

The reaming part of the proof is showing \pref{eq:rank1} and \eqref{eq:rank2} is equivalent to 
\begin{align}\label{eq:rank3}
      \rank( \Prr(\bar \Fb_t \mid \Hb_t) )= |\bar \Scal_t|. 
\end{align}
This is completed as follows. 

\paragraph{Part 1: \eqref{eq:rank3} implies \eqref{eq:rank1} and \eqref{eq:rank2} }

We have 
\begin{align*}
     |\bar \Scal_t|= \rank( \Prr(\bar \Fb_t \mid \Hb_t) ) &\leq \min(   \rank( \Prr(\bar \Fb_t \mid \bar \Sbb_t ) ),  \rank( \Prr(\bar \Sbb_t \mid \Hb_t ) ))\leq    |\bar \Scal_t|. 
\end{align*}
We use 
\begin{align*}
    \Prr(\bar \Fb_t \mid \Hb_t) = \Prr(\bar \Fb_t \mid \bar \Sbb_t)\Prr(\bar \Sbb_t \mid \Hb_t). 
\end{align*}
based on 
\begin{align*}
    \bar F_t \perp (H_t \setminus \bar H_t) \mid \bar H_t, S_t. 
\end{align*}


\paragraph{Part 2: \eqref{eq:rank1} and \eqref{eq:rank2} implies \eqref{eq:rank3}}

First, we have 
\begin{align*}
    \rank( \Prr(\bar \Fb_t \mid \Hb_t) ) &\leq \min(   \rank( \Prr(\bar \Fb_t \mid \bar \Sbb_t ) ),  \rank( \Prr(\bar \Sbb_t \mid \Hb_t ) ))=  |\bar \Scal_t|. 
\end{align*}
Second, 
\begin{align*}
    |\bar \Scal_t| &= \rank( \Prr(\bar \Fb_t \mid \bar \Sbb_t ) ) \\ 
       &= \rank( \Prr(\bar \Fb_t \mid \bar \Sbb_t ) )+\rank( \Prr(\bar \Sbb_t \mid \Hb_t ) ))-|\bar \Scal_t| \tag{From assumption}\\ 
       &\leq  \rank ( \Prr(\bar \Fb_t \mid \bar \Sbb_t ) \Prr(\bar \Sbb_t \mid \Hb_t ) )  ) \tag{Sylvester inequality}\\
       &= \rank(\Prr(\bar \Fb_t \mid \Hb_t) ). 
\end{align*}
Thus,
\begin{align*}
     \rank( \Prr(\bar \Fb_t \mid \Hb_t) )=|\bar \Scal_t|. 
\end{align*}


\section{Proof of \pref{sec:modeling}}

\subsection{Proof of \pref{thm:system_identification}}

The proof is completed by following \pref{thm:identify}. 

\subsection{Proof of Corollary \pref{cor:system_identification}}

Let $b^{[t]}_D(F_t) = \theta^{\top}_t \phi_{\Fcal}(F_t)$ where $\phi_{\Fcal}(F_t)$ is a one-hot encoding vector over $\Fcal_t$. Then, 
\begin{align*}
     \theta^{\top}_t B_t =  \theta^{\top}_{t+1} D_t.  
\end{align*}
Recall $B_t = \Prr(\Fb_t \mid \Hb_t), D_t = \EE[\rI(A_t=a_t,O_t=o_t)\mu_t(\bar H_t,A_t,O_t)\Fb_t \mid \Hb_t ]$. 

Let the SVD decomposition of $B_t $ be $A_1A_2A_3$ where $A_1 \in \RR^{|\Fcal_t|\times |\Scal| },A_2 \in \RR^{|\Scal|\times |\Scal| }, A_3 \in \RR^{|\Scal|\times |\Hcal_t| }  $. Here, from $\rank(\Prr(\Fb_t \mid \Hb_t))=|\Scal|$, $A_2$ is invertible. 
\begin{align*}
    I = A^{\top}_1 B_t A^{\top}_3 A^{-1}_2 = A^{\top}_1 \Prr(\Fb_t \mid \Sbb_t)\Prr(\Sbb_t \mid \Hb_t) A^{\top}_3 A^{-1}_2. 
\end{align*}
Therefore, we have
\begin{align*}
     A^{\top}_1 \Prr(\Fb_t \mid \Sbb_t) =  \{\Prr(\Sbb_t \mid \Hb_t) A^{\top}_3 A^{-1}_2\}^{-1} 
\end{align*}
noting $\Prr(\Sbb_t \mid \Hb_t) A^{\top}_3 A^{-1}_2$ is full-rank. 

Thus, 
\begin{align*}
       \theta^{\top}_t B_t \{A^{\top}_3 A^{-1}_2\}=\theta^{\top}_t \Prr(\Fb_t \mid \Sbb_t)\Prr(\Sbb_t \mid \Hb_t) A^{\top}_3 A^{-1}_2
\end{align*}
and
\begin{align*}
    \theta^{\top}_{t+1} D_t\{A^{\top}_3 A^{-1}_2\}= \theta^{\top}_{t+1}\EE[\rI(A_t=a_t,O_t=o_t)\mu_t(\bar H_t,A_t,O_t)\Fb_t \mid \Sbb_t ]\Prr(\Sbb_t \mid \Hb_t) A^{\top}_3 A^{-1}_2. 
\end{align*}
Since $\Prr(\Sbb_t \mid \Hb_t) A^{\top}_3 A^{-1}_2$ is invertible, we have
\begin{align*}
      \theta^{\top}_t \Prr(\Fb_t \mid \Sbb_t)= \theta^{\top}_{t+1}\EE[\rI(A_t=a_t,O_t=o_t)\mu_t(\bar H_t,A_t,O_t)\Fb_t \mid \Sbb_t ] 
\end{align*}
Noting $ \Prr(\Fb_t \mid \Sbb_t)$ is full-column rank, we obtain 
\begin{align*}
      \theta^{\top}_t = \theta^{\top}_{t+1}\EE[\rI(A_t=a_t,O_t=o_t)\mu_t(\bar H_t,A_t,O_t)\Fb_t \mid \Sbb_t ]\Prr(\Fb_t \mid \Sbb_t)^{+}. 
\end{align*}
Noting $ \Prr(\Sbb_t \mid \Hb_t)$ is full-raw rank, we obtain 
\begin{align*}
      \theta^{\top}_t &= \theta^{\top}_{t+1}\EE[\rI(A_t=a_t,O_t=o_t)\mu_t(\bar H_t,A_t,O_t)\Fb_t \mid \Sbb_t ]\Prr(\Sbb_t\mid \Hb_t)\Prr(\Sbb_t\mid \Hb_t)^{+} \Prr(\Fb_t \mid \Sbb_t)^{+} \\ 
      &= \theta^{\top}_{t+1}\EE[\rI(A_t=a_t,O_t=o_t)\mu_t(\bar H_t,A_t,O_t)\Fb_t \mid \Sbb_t ]\Prr(\Sbb_t\mid \Hb_t)\Prr(\Sbb_t\mid \Hb_t)^{+} \Prr(\Fb_t \mid \Sbb_t)^{+} \\ 
       &= \theta^{\top}_{t+1}\EE[\rI(A_t=a_t,O_t=o_t)\mu_t(\bar H_t,A_t,O_t)\Fb_t \mid \Hb_t ] \Prr(\Fb_t \mid \Hb_t)^{+}. 
\end{align*}

\section{Proof of \pref{sec:finite}}

\subsection{Proof of \pref{thm:bellman}}
We refer it to the proof of ----. 

\subsection{Proof of  \pref{thm:final_error} }
Recall using telescoping sum, we have 
\begin{align*}
   & J(\pi^e) - \EE[\hat b^{[0]}_V(F_0)  ] \\
   &=  J(\pi^e)-\EE[\hat b^{[0]}_V(F_0)  ]  \\ 
   &+  \sum_{t=0}^{H-1} \EE[\EE[ \nu_{t-1} \mid  H_t,S_t] \mu_{t}(\bar H_t,A_t,O_t)\gamma \hat b^{[t+1]}_V(\bar H_{t+1},F_{t+1})  -  \gamma\EE[ \nu_{t} \mid  \bar H_{t+1}, S_{t+1}] \hat b^{[t+1]}_V(\bar H_{t+1},F_{t+1})   ] \\
  &= \sum_{t=0}^{H-1} \gamma^t \EE\bracks{\EE[ \nu_{t-1}\mid  \bar H_t,S_t]\braces{\EE[\mu_t(\bar H_t,O_t,A_t)\{R_t+ \gamma \hat b^{[t+1]}_V(\bar H_{t+1},F_{t+1})\}- \hat b^{[t]}_V(\bar H_t,F_t)  \mid \bar H_t, S_t] } }. 
\end{align*}
Then, from CS inequality, the error is upper bounded by 
\begin{align*}
   & \sum_{t=0}^{H-1} \gamma^t \EE\bracks{\EE[ \nu_{t-1}\mid  \bar H_t,S_t]^2}^{1/2} \EE\bracks{\braces{\EE[\mu_t(\bar H_t,O_t,A_t)\{R_t+ \gamma \hat b^{[t+1]}_V(\bar H_{t+1},F_{t+1})\}- \hat b^{[t]}_V(\bar H_t,F_t)  \mid \bar H_t, S_t] }^2 }^{1/2} \\
    &=  \sum_{t=0}^{H-1} \gamma^t \EE\bracks{\frac{d^{\pi^e}_t(\bar H_t,S_t)^2 }{d^{\pi^b}_t(\bar H_t,S_t)^2} }^{1/2} \EE\bracks{\{\Tcal^{\Scal}_t(\hat f_t,\hat f_{t+1})(\bar H_t,S_t)\}^2 }^{1/2} \\
\end{align*}


\section{Proof of \pref{sec:without_completeness}}

We have 
\begin{align*}
   &J(\pi_e) =   \EE[\sum_{t=0}^{H-1}  \gamma^t\nu_t R_t]  =   \EE[\sum_{t=0}^{H-1}\EE[ \nu_{t-1} \mid  \bar H_t,S_t]  \mu_t(\bar H_t,O_t,A_t) \gamma^t R_t] \tag{$(U_{t} \setminus \bar H_t )  \perp A_t,R_t,O_t \mid S_t,\bar H_t$} \\ 
    &=   \EE[\sum_{t=0}^{H-1}\EE[ b^{[t]}_W(H^{\diamond}_t )\mid  \bar H_t,S_t]  \mu_t(\bar H_t,O_t,A_t) \gamma^t R_t] \tag{Existence of weight bridge functions}\\ 
     &=   \EE[\sum_{t=0}^{H-1} b^{[t]}_W(H^{\diamond}_t )  \mu_t(\bar H_t,O_t,A_t) \gamma^t R_t] \\ 
    &=   \EE[\sum_{t=0}^{H-1} \gamma^t b^{[t]}_W(H^{\diamond}_t )  \mu_t(\bar H_t,O_t,A_t) \EE[ R_t \mid H_t]] \tag{$R_t  \perp O_t,A_t,H^{\diamond}_t \mid H_t $ }\\ 
 \end{align*}  
Thus, 
{\small 
 \begin{align*}
     &J(\pi_e)  =  \sum_{t=0}^{H-1} \gamma^t \EE[ b^{[t]}_W(H^{\diamond}_t )\{- \EE[\mu_t(\bar H_t,O_t,A_t)\gamma b^{[t+1]}_V(\bar H_{t+1},F_{t+1})+ b^{[t]}_V(\bar H_t,F_t)  \mid H_t] \} ]  \\ 
     &= \EE[b^{[0]}_V(F_0)  ] +\\
         & \sum_{t=0}^{H-1}\gamma^t \EE \bracks{ - b^{[t]}_W(H^{\diamond}_t ) \EE[\mu_t(\bar H_t,O_t,A_t)\gamma b^{[t+1]}_V(\bar H_{t+1},F_{t+1}) \mid H_t] + \gamma b^{[t+1]}_W(H^{\diamond}_{t+1} ) \EE[b^{[t+1]}_V(\bar H_{t+1},F_{t+1})  \mid H_{t+1}]  } \tag{Telescoping sum} \\ 
    &= \EE[b^{[0]}_V(F_0)  ] \\
         & +\sum_{t=0}^{H-1}\gamma^t \EE\bracks{-b^{[t]}_W(H^{\diamond}_t ) \mu_{t}(\bar H_t,O_t,A_t)\gamma b^{[t+1]}_V(\bar H_{t+1},F_{t+1})  +  \gamma b^{[t+1]}_W(H^{\diamond}_{t+1} ) b^{[t+1]}_V(\bar H_{t+1},F_{t+1})   } . 
\end{align*}
}
In the last line, we use $H^{\diamond}_t \perp (A_t,O_t,F_{t+1},\bar H_{t+1} )\setminus \bar H_t \perp H_t $ and $ H^{\diamond}_{t+1} \perp F_{t+1} \mid H_{t+1}$. Here,
\begin{align*}
    & \EE[\EE[ b^{[t]}_W(H^{\diamond}_t ) \mu_{t}(\bar H_t,A_t,O_t) b^{[t+1]}_V(\bar H_{t+1},F_{t+1})] \\
    &=\EE[\EE[ \EE[b^{[t]}_W(H^{\diamond}_t )\mid \bar H_t,S_t] \mu_{t}(\bar H_t,A_t,O_t) b^{[t+1]}_V(\bar H_{t+1},F_{t+1})] ] \tag{$H^{\diamond}_t   \perp (A_t,O_t,F_{t+1},\bar H_{t+1} )\setminus \bar H_t \mid  \bar H_t,S_t $} \\
   &=\EE[\EE[ \EE[\nu_t \mid \bar H_t,S_t] \mu_{t}(\bar H_t,A_t,O_t) b^{[t+1]}_V(\bar H_{t+1},F_{t+1})] \tag{Definition} \\
    &=\EE[\EE[ \nu_{t} \mid  \bar H_{t+1}, S_{t+1}] b^{[t+1]}_V(\bar H_{t+1},F_{t+1})   ] \tag{See proof of \pref{thm:identify}}\\ 
     &=\EE[\EE[ b^{[t+1]}_W(H^{\diamond}_{t+1} ) \mid  \bar H_{t+1}, S_{t+1}] b^{[t+1]}_V(\bar H_{t+1},F_{t+1})   ] \tag{Definition}\\
     &= \EE[b^{[t+1]}_W(H^{\diamond}_{t+1} )b^{[t+1]}_V(\bar H_{t+1},F_{t+1})   ].  \tag{ $H^{\diamond}_{t+1}   \perp F_{t+1}  \mid  \bar H_{t+1},S_{t+1} $}
\end{align*}
Thus, $J(\pi_e) = \EE[b^{[0]}_V(F_0)  ] $. 
